Smart Conversational Agents for Reminiscence

In this paper we describe the requirements and early system design for a smart conversational agent that can assist older adults in the reminiscence process. The practice of reminiscence has well documented benefits for the mental, social and emotional well-being of older adults. However, the technology support, valuable in many different ways, is still limited in terms of need of co-located human presence, data collection capabilities, and ability to support sustained engagement, thus missing key opportunities to improve care practices, facilitate social interactions, and bring the reminiscence practice closer to those with less opportunities to engage in co-located sessions with a (trained) companion. We discuss conversational agents and cognitive services as the platform for building the next generation of reminiscence applications, and introduce the concept application of a smart reminiscence agent.

==> sections/bot-algorithm.tex <==
#  User     K   = Knowledge acquired about the user
#           L   = Missing knowledge (latent)
#           Mod = User moderators
#  Memento  Km  = Knowledge acquired about the memento
#           Lm  = Missing knowledge (latent)            
#           Mod_m = User moderators in the session

process_turn(trigger, input):
begin

   // We process the input provided by the user
   // in response to the trigger
   Tt       := extract_information(input)
   (Kt, Lt) := consolidate_knowledge(trigger, Tt)   
   
   // Infer relevant user session “moderators”
   // such as sentiment, feeling, engagement   
   Mod_t := infer_moderators(Mod_m, input) 
   
   // Compute the gain of this turn, in relation to
   // the utility (knowledge) and user response (Mod_t)
   v_t := gain(Kt, Mod_t)
   
   // See what potential triggers we could use next
   Q := related_triggers(Kt, Lt, Km, Lm, K, L)   
   
   // Estimate the gain of poential triggers, and select
   // the one with more potential
   G := apply(estimate_gain, Q, Mod_t, Mod, trigger, v_t)
   next_trigger := Q [max (G)]
   
   // We paraphrase the trigger according to the 
   // user moderators   
   t := instantiate_trigger(next_trigger, Mod_t, Mod)
   
   return t
end

==> sections/sveta-agents.tex <==
\subsection{Conversational agents}

{\color{red} Sveta: Please work on this section.}

\paragraph{Definition}

"Conversational AI is the study of techniques for software agents that can engage in natural conversational interactions with humans" [alexa prize ref.,2017].
%"A chatbot is an example of a text-based conversational agent".
First introduced in 1960 \cite{Weizenbaum66}, the technology of conversational agents nowadays getting widespread popularity by allowing humans to communicate in a natural way with computer systems. 

Main concepts that conversational agents operate with are: an Intent, Entity; Action and Conversation/Story. 
"An intent represents a mapping between what a user says and what action should be taken by your software" \cite{DialogFlow}.
"Entities" are keywords recognized by nlu and "actions" are the activities that can be performed by the system.
\paragraph{Platforms}
Several leading tech companies have proposed solutions of platforms for fast chatbots building from scratch such as Wit.ai (facebook), DialogFlow (amazon), watson (IBM) and others.
%\paragraph{Dialog management}
%\paragraph{Limitations}
\paragraph{Aims}
Conversational agents can be generally separated to task-based, informational and conversational  categories.

Task-based or transactional bots are aimed at executing the action requested by the user in natural language such as booking a hotel (SnapTravel, Guardian).

Informational bots are providing the information on the topic asked by user (Guardian, CRQA), while conversational bots are able to  support conversation on the general topics (Chrous) \cite{lasecki2013chorus}.

From the perspective of domain, agents can be  separated to generic, which are able to communicate on multiple general topics (Chrous) and domain specific, such as Woebot, recent chatbot recently developed in Stanford and aimed at depression treatment and applying  cognitive behaviour therapy (CBT) through conversation with user \cite{fitzpatrick2017delivering}.

To our knowledge, there is no conversational agent yet developed to support reminiscence therapy sessions.

==> sections/sveta-metrics.tex <==
\textbf{Engagement} Engagement describes the level of involvement and interest of a person in the conversation. Capturing engagement is important as it has shown to be associated with longer conversations and higher sentiment score \cite{cervoneroving}.
Different engagement metrics have been proposed for conversational agents, such as: 
i) \textit{conversation length}, in minutes and/or amount of dialog turns \cite{fitzpatrick2017delivering,cervoneroving}; 
ii) \textit{total number of interactions} with the bot over period of session \cite{fitzpatrick2017delivering};
iii) subjective \textit{user engagement ratings} \cite{cervoneroving};
iv) cumulative \textit{average sentiment score}, to see the user sentiment towards a topic \cite{cervoneroving}.

%\textbf{Acceptability and usability} can be measured with \textit{self-reported questionnaires} and usually designed by researchers for specific study goals and include overall questions on satisfaction with technology and the user intent to continue use the technology \cite{fitzpatrick2017delivering}.

\textbf{Task completion} measure is displaying whether the goal of interaction was achieved such as e.g flight or hotel booked for user \cite{SnapTravel}. 

For the  case of the reminiscence bot the task-specific goal will be to collect maximum \textit{relevant information about the user}: amount of content which the user has provided during one conversation session (amount of pictures uploaded, amount of relevant person-related data attributes filled out)

The metrics that have been recently proposed for the task-based evaluation are: 
i) \textit{task completion rate} and ii) \textit{completion time}, which can be measured as a number of dialog turns the user talks to bot to complete a task \cite{huang2015guardian}.

\textbf{Conversation quality}
 describes how much consistent the conversation is and the ability of bot correctly remembering things the user said on the previous turns of conversation.

For evaluation of conversation quality several metrics has been proposed : i) conversational consistency, ii ) memory of past events, iii) response speed (has been applied for crowd-empowered bots)\cite{lasecki2013chorus}

\textbf{Human-like communication}
Other researches take human-like communication as a measure for the conversation quality and analyse conversation logs content to see if user conversate with bot as with a human, e.g. using greetings, showing "proactivity"\cite{kopp2005conversational}.
